A General Family of Trimmed Estimators for Robust High-dimensional Data Analysis

We consider the problem of robustifying high-dimensional structured estimation. Robust techniques are key in real-world applications which often involve outliers and data corruption. We focus on trimmed versions of structurally regularized M-estimators in the high-dimensional setting, including the popular Least Trimmed Squares estimator, as well as analogous estimators for generalized linear models and graphical models, using possibly non-convex loss functions. We present a general analysis of their statistical convergence rates and consistency, and then take a closer look at the trimmed versions of the Lasso and Graphical Lasso estimators as special cases. On the optimization side, we show how to extend algorithms for M-estimators to fit trimmed variants and provide guarantees on their numerical convergence. The generality and competitive performance of high-dimensional trimmed estimators are illustrated numerically on both simulated and real-world genomics data.

==> its_analysis_copy.tex <==
 
We now focus on the special case of high-dimensional linear regression, and apply Theorem \ref{ThmGeneral} to problem \eqref{EqnRobustLS}.  In particular, 
if $i \in G$,
%\begin{align*}%\label{EqnLinearModel}
	$y_i = \inner{x_i}{\Ttheta} + \epsilon_i$ 
%\end{align*}
where the observation noise $\epsilon_i$ follows zero mean and has sub-Gaussian tails. Otherwise, for $i \in B$,
%\begin{align*}%\label{EqnLinearModel}
	$y_i = \inner{x_i}{\Ttheta} + \delta_i$
%\end{align*}
where $\delta_i$ is the amount of arbitrary corruption. 

% We show that by Theorem \ref{ThmOpt}, the robustified version of ISTA using partial minimization, preserves the convergence properties of standard ISTA, with an additional cost of sorting $n$ items at every update iteration:
%\begin{corollary}\label{CorLSOpt}
%Let $\{\theta^{(t)}\}$ and $\{w^{(t)}\}$ be the sequences for parameters $\theta$ and $w$ generated by Algorithm \ref{alg:trimmedGeneral} for high-dimensional linear models. Suppose that the largest eigenvalue of $X^\top X/n$, $\lambda_{\max}(X^\top X/n)$, is bounded by some constant $L$. Then, these algorithms with $\eta^{(t)} := 1/L$ are guaranteed to converge to a local optimum $(\Ltheta,\Lw)$. Moreover, for any $t \geq 1$, 
%\begin{align*}
%	F(\theta^{(t)},w^{(t)}) - F(\Ltheta,\Lw) = O(1/t)
%\end{align*}
%where $F(\theta,w)$ is the objective of \eqref{EqnRobustLS}. %$c(n)$ is a cost for sorting $n$ items.
%\end{corollary}
% 
%The proof is relegated to the supplementary materials.
%While we only focus on standard proximal gradient method, other faster methods can be robustified for solving partial minimization like \eqref{EqnRobustGeneral3} preserving the convergence properties of original methods. For example, it can be shown that the convergence properties (the fast global convergence under restricted smoothness condition) of the composite gradient descent for non-convex estimation \cite{LW15} can be preserved in the partial minimization.
%
%
%Now we apply Theorem \ref{ThmGeneral} to the problem \eqref{EqnRobustLS} and 
In order to derive an actual bound from the general framework of Theorem \ref{ThmGeneral}, we consider the following natural setting, which has been widely studied in past work on conventional high dimensional linear models: 
%\begin{enumerate}[leftmargin=0.1cm, itemindent=1.1cm,label=\textbf{(C-$\bf{4}$)}, ref=\textnormal{(C-$4$)}]
%	\item $\|\Ttheta\|_0 := |\{\Ttheta_j \, : \, \Ttheta_j \neq 0 \, \text{ for } j=1,\hdots,p\}| \leq k$. \label{Con:Sparsity}  
%\end{enumerate}
\begin{enumerate}[leftmargin=0.5cm, itemindent=2cm,label=\textbf{(LTS1)}, ref=\textnormal{(LTS1)}]
	\item {\bf ($\Sigma$-Gaussian ensemble)} Each sample $x_i$ is i.i.d. sampled from $N(0,\Sig)$. \label{ConLS:XGauss}
\end{enumerate}
\vspace{-.3cm}
\begin{enumerate}[leftmargin=0.5cm, itemindent=2cm,label=\textbf{(LTS2)}, ref=\textnormal{(LTS2)}]
	\item {\bf (Sub-Gaussian noise)} The noise vector $\epsilon \in \reals^n$ is zero-mean and has sub-Gaussian tails, which means that for any fixed vector $v$ such that $\|v\|_2 = 1$, 
%\begin{align*}
	$\P\left[|\inner{v}{\epsilon}| \geq t\right] \leq 2 \exp \left(-\frac{t^2}{2\sigma^2}\right)$ for all $t >0$.
%\end{align*}
	The sub-Gaussian is quite a wide class of distributions, and contains the Gaussian family as well as and all bounded random variables.  
\label{ConLS:NsubGauss}
\end{enumerate}
\vspace{-.3cm}
\begin{enumerate}[leftmargin=0.5cm, itemindent=2cm,label=\textbf{(LTS3)}, ref=\textnormal{(LTS3)}]
	\item {\bf (Column normalization)} Let $X \in \reals^{n \times p}$ be the design matrix whose $i$-th row is the covariate $i$-th sample: $x_i^\top$, and $X^j\in \reals^n$ be the $j$-th column vector of $X$. Then, $\frac{\|X^j\|_2}{\sqrt{h}} \leq 1$. As pointed out in \citet{NRWY12}, we can always rescale linear models with out loss of generality to satisfy this condition. \label{ConLS:colNorm}
\end{enumerate}
The following assumptions are required for our estimator to be resilient to outliers and strongly consistent:
%
\begin{enumerate}[leftmargin=0.5cm, itemindent=1.8cm,label=\textbf{(C-$\bf{h}$)}, ref=\textnormal{(C-$h$)}]
	%\item $\Loss_{(i)}(\theta^*;y_i,x_i) \geq r_{\min}\geq 0$ for all $i \in B$.\label{Con:Bad}
	\item Let $h$ be the number of good samples: $|G| = h$ and hence $|B| = n-h$. Then, we assume that larger portion of samples are genuine and uncorrupted so that $\frac{|G|-|B|}{|G|} \geq \alpha$ where $0 < \alpha \leq 1$. If we assume that 40\% of samples are corrupted, then $\alpha = 1/3$. \label{Con:h}  
\end{enumerate}
\begin{enumerate}[leftmargin=0.5cm, itemindent=2cm,label=\textbf{(LTS4)}, ref=\textnormal{(LTS4)}]
	\item \change{We set the tuning parameter $\rho$ in \eqref{EqnRobustLS} as $\rho \leq \frac{C_1}{2} \sqrt{\frac{h}{\log p}}$ for some constant $C_1$. This setting requires that the number of good samples $h$ is larger than or equal to $\big(\frac{2k\|\Ttheta\|_\infty}{C_1}\big)^2 \log p$ so that the true regression parameter $\Ttheta$ is feasible for the objective.}\label{ConLS:R}
%	\item The problem \eqref{EqnRobustLS} has a constraint of $g(\theta) \leq \rho$ where $g(\Ttheta) \leq \rho$. Here we assume that $\rho \leq \frac{C_1}{2} \sqrt{\frac{h}{\log p}}$ for some constant $C_1$. When $g(\cdot)$ is set to $\|\cdot\|_1$, this requires $\|\Ttheta\|_1 \leq \frac{C_1}{2} \sqrt{\frac{h}{\log p}}$. If $\|\Ttheta\|_2 \leq c$ for example, this condition can be satisfied by setting $C_1$ as $2c\sqrt{\log p}$ since $\|\Ttheta\|_1 \leq \sqrt{k}\|\Ttheta\|_2 \leq c\sqrt{k}$. \label{ConLS:R}
\end{enumerate}
%%%%%%%%%%%%%%%%%%%%%
%\vspace{-.3cm}
%\begin{enumerate}[leftmargin=0.2cm, itemindent=2.6cm,label=\textbf{(C-Corrupt)}, ref=\textnormal{(C-Corrupt)}]
%	\item We also require the \emph{identifiability} condition for the model \eqref{EqnLinearModels}. \change{Intuitively it is impossible to recover the true signal by a trimming approach when the amount of corruptions exceed that of normal observation errors.} Therefore, for true regression parameter $\Ttheta$, the squared loss for bad samples (by corruptions), which is at most $(\max_{i}\delta_i^2) |B|$, is smaller than or equal to squared loss for good samples (by observation errors): $(\max_{i}\delta_i^2) |B| \leq C^2_2 h$ for some small constant $C_2$. \change{Here without loss of generality, we can assume that $\max_{i}\delta_i^2$ is bounded by some constant since we can always rescale the linear models properly without changing the signal $\theta$}.\label{ConLS:MaxCorrupt}
%\end{enumerate}
%
%\vspace{-.2cm}
%%%%%%%%%%%%
%\textcolor{red}{GOT RID OF PROBLEMATIC C-Corrupt and put definition of constant $C_2$ in the body.}
Under these conditions, we can recover the following error bounds of high-dimensional LTS \eqref{EqnRobustLS}, as a corollary of Theorem \ref{ThmGeneral}:
\begin{corollary}\label{Cor:LS}
	Consider corrupted linear models \eqref{EqnLinearModels} when $\|\Ttheta\|_0 \leq k$. Suppose that  conditions \ref{Con:h}, \ref{ConLS:XGauss}, \ref{ConLS:NsubGauss}, \ref{ConLS:colNorm}, and \ref{ConLS:R} hold. \change{Also suppose that we  find a local minimum $(\Ltheta,\Lw)$ of \eqref{EqnRobustLS},  choosing }
	\begin{align*}
		\lambda = \Big(c \, C_1 \max_{j=1,\hdots,p} \Sig_{jj} + c' \,C_2 \sqrt{\matNorm{\Sig}_2} \Big) \sqrt{\frac{\log p}{h}}
	\end{align*}
	where $\matNorm{\Sig}_2$ is the largest singular value of $\Sig$, $C_2$ is a constant such that $ C^2_2 \geq \frac{(\max_{i}\delta_i^2) |B|}{h}$ and $c$ and $c'$ are some positive constants.\footnote{Here without loss of generality, we can assume that $\max_{i}\delta_i^2$ is bounded by some constant since we can always rescale the linear models properly without changing the signal $\theta$.} \change{Then, $(\Ltheta,\Lw)$ is guaranteed to satisfy \ref{Con:rsc} and \ref{Con:inc} for the specific case of \eqref{EqnRobustLS}, and have the following error bounds:} for $C'_1 := c \, C_1 \max_{j=1,\hdots,p} \Sig_{jj}$ and $C'_2 := c' \,C_2 \sqrt{\matNorm{\Sig}_2}$,
\begin{align*}
	\|\Ltheta - \Ttheta\|_2 \leq \, & \frac{1}{\RSCcon}\bigg( (C'_1 + C'_2) \sqrt{\frac{k \log p}{h}} + C'_2 \sqrt{\frac{|B|\log p}{h}} \bigg) \, , \nonumber\\
	\|\Ltheta - \Ttheta\|_1 \leq \, & \frac{1}{\lambda\, \RSCcon}\bigg( C''_1 \sqrt{\frac{k \log p}{h}} + C'_2 \sqrt{\frac{|B|\log p}{h}}\bigg)^2 
\end{align*}
with probability at least $1-c_1 \exp(-c_1' h \lambda^2)$ for some universal positive constants $c_1$ and $c'_1$.
\end{corollary}

\textcolor{red}{TODO: Is this $C''_1$ or $C'_1$?}

%Note that the error bounds derived in Theorem \ref{Thm:LS} and hence in Corollary \ref{Cor:LS} are applicable to any local optimum satisfying the first order stationary condition of the problem \eqref{EqnRobustLS}. 

\change{Note that Corollary \ref{Cor:LS}  concerns any \emph{single} {local minimum. %  derived by any optimization algorithm guaranteed to converge to a local optimum. %since all local optima \emph{are not} required to be guaranteed simultaneously. 
For the guarantees of \emph{multiple} local optima simultaneously, we may use a union bound from the corollary.}}

\paragraph{Remarks.}
It is instructive to compare the error rates and conditions in Corollary \ref{Cor:LS} with statistical guarantees of extended Lasso analyzed in \citet{Nguyen2011b}. The extended Lasso estimator solves:
\begin{align*}%\label{EqnExtendedLasso}
	\minimize_{\theta,e} \ &  \frac{1}{2n}\sum_{i=1}^{{n}} \big(y_i - \inner{x_i}{\theta} - e_i \big)^2 + \lambda_\theta \|\theta\|_1 + \lambda_e \|e\|_1 
\end{align*}
where $\lambda_e$ is the regularization parameter for parameter $e$ capturing corruptions.  $e$ is encouraged to be sparse to reflect the fact that only a fraction of samples is corrupted.
The $\ell_2$ norm-based error rate in Corollary \ref{Cor:LS} is almost the same as that of extended Lasso: $\|\widehat{\theta}_{\text{E\_Lasso}} - \Ttheta\|_2 = O\Big(\sqrt{\frac{k\log p}{n}} + \sqrt{\frac{|B| \log n}{n}}\Big)$ under the standard Gaussian design setting \ref{ConLS:XGauss}. As long as at least a linear fraction of samples is not contaminated (that is, $h \geq \alpha n$ for $\alpha \in (0,1] $), $1/h \leq 1/(\alpha n)$ the error rates for both estimators will be asymptotically the same.  

However, it is important to revisit the conditions required for the statistical guarantees of extended Lasso. Besides an extended version of the restricted eigenvalue condition, \citet{Nguyen2011b} assumes a mutual incoherence condition, which in turn requires $c \sqrt{\matNorm{\Sig}_2}\max\Big\{\frac{k}{|B|},\frac{|B|}{k}\Big\} \Big(\sqrt{\frac{k}{n}} + \sqrt{\frac{|B|}{n}} + \sqrt{\frac{\log p}{n}}\Big) \leq \frac{1}{16}$ for some large and fixed constant $c$. Provided that $k$ and $|B|$ are fixed, the inequality can hold for a large enough sample size $n$. However, when $|B|$ grows with $n$, this condition will be violated; for example if (i) a square root fraction of samples is corrupted ($|B| = \alpha \sqrt{n}$) for a fixed $k$ or (ii) a linear fraction of $n$ is corrupted ($|B| = \alpha n$), then $c' \sqrt{\matNorm{\Sig}_2}$ can easily exceed $1/16$. Our experimental results of Section~\ref{sec:exps} will confirm this observation: as the fraction of corruptions increases, the performance of extended Lasso deteriorates compared to that of our estimator \eqref{EqnRobustLS}.


%As an another example of using Theorem \ref{ThmGeneral} for corrupted linear models, an additional corollary is provided in the appendix for the case of corrupted covariates. 

%Other corrolaries instantiating Theorem \ref{ThmGeneral} can be derived similarly, e.g. for generalized linear models and other structures.

%\todo{[TODO] add some texts on extending to GLMs}


\paragraph{Statistical Guarantees When Covariates Are Corrupted.}
In the linear model \eqref{EqnLinearModels}, corruption is considered in the space of the response variable $y_i \in \reals$: namely an additional random variable $\delta_i \in \reals$ is used to model corruption in the response space. Even in the case where we have outliers with corrupted covariates $x_i + \delta' \in \reals^p$, $\delta_i$ can be understood as the mean-shift variable to model $\inner{\delta'}{\Ttheta}$. For linear models, modeling outliers in the parameter space or modeling them in the output space is thus equivalent (In constrast, for more general GLM settings, the link function is not the identity function and both approaches are distinct, see e.g. \citep{YTR13}). Nevertheless, when outliers stem from corrupted covariates, condition \ref{ConLS:XGauss} might be violated. 
For this setting, we introduce the following alternative condition:
\begin{enumerate}[leftmargin=0.5cm, itemindent=2cm,label=\textbf{(LTS5)}, ref=\textnormal{(LTS5)}]
	\item {\bf ($\Sigma$-Gaussian ensemble)} Each sample $x_i$ in $G$ is i.i.d. sampled from $N(0,\SigG)$. Let $X^B$ be the sub-design matrix in $\reals^{|B|\times p}$ corresponding to outliers. Then, we define $f(X^B)$ such that $\matNorm{X^B}_2 \leq f(X^B) \sqrt{|B| \log p}$. \label{ConLS:XCor}
\end{enumerate}
Under condition \ref{ConLS:XCor} we recover results similar to Corollary \ref{Cor:LS}:
\begin{corollary}\label{Cor:XCor}
	Consider linear models in \eqref{EqnLinearModels} where $\|\Ttheta\|_0 \leq k$. Suppose that all the conditions \ref{Con:h}, \ref{ConLS:NsubGauss}, \ref{ConLS:colNorm}, \ref{ConLS:R} and \ref{ConLS:XCor} hold. Also suppose that we choose the regularization parameter 
	\begin{align*}
		\lambda = \Big(c \, C_1 \max_{j=1,\hdots,p} \Sig_{jj} + c' \,C_2 f(X^B) \Big) \sqrt{\frac{\log p}{h}}\, 
	\end{align*}
	where $C_2$ is a constant such that $ C^2_2 \geq \frac{(\max_{i}\delta_i^2) |B|}{h}$ and $c$ and $c'$ are some positive constants.
	
	Then, defining $C'_1 := c \, C_1 \max_{j=1,\hdots,p} \Sig_{jj}$, and $C'_2 := c' \,C_2 f(X^B)$, {any local minimum of \eqref{EqnRobustLS}} is guaranteed to have the following error bounds:
\begin{align*}
	\|\Ltheta - \Ttheta\|_2 \leq \, & \frac{1}{\RSCcon}\bigg( (C'_1 + C'_2) \sqrt{\frac{k \log p}{h}} + C'_2 \sqrt{\frac{|B|\log p}{h}} \bigg) \, , \nonumber\\
	\|\Ltheta - \Ttheta\|_1 \leq \, & \frac{1}{\lambda\, \RSCcon}\bigg( C''_1 \sqrt{\frac{k \log p}{h}} + C'_2 \sqrt{\frac{|B|\log p}{h}}\bigg)^2 
\end{align*}
with probability at least $1-c_1 \exp(-c_1' h \lambda^2)$ for some universal positive constants $c_1$ and $c'_1$.
\end{corollary}

\textcolor{red}{TODO: Is this $C''_1$ or $C'_1$?}




























==> table1.tex <==
\begin{table}[t!]
	\footnotesize
	\caption{Average performance measures for comparison methods on simulated data under sparse linear models with contamination scenario (S1). Comparison methods are evaluated in terms of the parameter estimation error ($\ell_2$ error) and the sparsity pattern recovery (true positive rate (TPR) and false positive rate (FPR)) } \label{ta::expresults1}
	%\begin{center}
	\centering
%	\begin{tabular}{|c|cccc|}
%	\hline
%Contamination 5\% & L2 error & Linf error & TPR & FPR\\
%\hline
%Lasso & 12.50 & 2.7234 & 0.41 & 0.21\\
%LAD-Lasso & 7.38 & 1.2547 & 0.64 & 0.29\\
%Extended Lasso &  6.39 & 1.15 & 0.70 & 0.21\\
%ROMP & 7.69 & 1.97 & 0.67 & 0.24\\
%LTS & 5.80 & 0.98 & 0.76 & 0.27\\
%	\hline
%\end{tabular}
%\begin{tabular}{cc}
\begin{tabular}{c|ccc}
%\hline
\abovespace\belowspace
Contamination 10\% & $\ell_2$ error &  TPR & FPR\\
\hline
Lasso & 17.23 &  0.62 & 0.35\\
LAD-Lasso & 8.87 & 0.63 & 0.27\\
Extended Lasso & 8.86 & 0.60 & 0.19\\
ROMP & 11.47& 0.46 & 0.24\\
{\bfseries Sparse-LTS} & 8.09 & 0.70& 0.17\\
\belowspace
{\bfseries Sparse-LTS-Ada} &  8.01 & 0.71  & 0.16  \\
\hline
\end{tabular}
%	
%	\begin{tabular}{|c|cccc|}
%	\hline
%Contamination 20\% & L2 error & Linf error & TPR & FPR\\
%		\hline
%Lasso & 18.23 & 4.04 & 0.45 & 0.54\\
%LAD-Lasso & 11.97 & 2.35 & 0.59 & 0.43\\
%Extended Lasso & 12.44 & 2.94 & 0.50 & 0.44\\
%ROMP & 12.42 & 2.95 & 0.56& 0.55\\
%LTS & 9.23 & 1.74 & 0.66 & 0.31\\
%		\hline
%\end{tabular}
%& 
\begin{tabular}{c|ccc}
%\hline
\abovespace\belowspace
Contamination 30\% & $\ell_2$ error & TPR & FPR\\
\hline
Lasso & 38.23  & 0.33 & 0.24\\
LAD-Lasso & 14.093 &  0.50 & 0.29\\
Extended Lasso & 13.63 & 0.58 & 0.29\\
ROMP & 32.42 &  0.56& 0.55\\
{\bfseries Sparse-LTS} & 11.23 &  0.60 & 0.25\\
\belowspace
{\bfseries Sparse-LTS-Ada} &  10.73 & 0.62 & 0.25 \\
\hline
\end{tabular}
%\end{tabular}

%\end{center}
\end{table}


==> table2.tex <==
\begin{table}[t!]
	\footnotesize
	\caption{Average performance measures for comparison methods on simulated data under sparse linear models with contamination scenario (S2).} \label{ta::expresults2}
	%\begin{center}
	\centering
	%\begin{tabular}{cc}
	\begin{tabular}{c|ccc}
	%\hline
	\abovespace\belowspace
	Contamination 10\% & $\ell_2$ error &  TPR & FPR\\
	\hline
	Lasso & 34.37 & 0.52 & 0.49 \\
	LAD-Lasso & 21.04 & 0.42 & 0.40\\
	Extended Lasso & 13.71 & 0.66  &0.22 \\
	ROMP & 40.25 &0.46 & 0.39\\
	{\bfseries Sparse-LTS} & 10.52 & 0.83 & 0.22\\
	\belowspace
	{\bfseries Sparse-LTS-Ada} &  10.37  &   0.81&  0.20 \\
	\hline
	\end{tabular}
	%&
	\begin{tabular}{c|ccc}
	%\hline
	\abovespace\belowspace
	Contamination 30\% & $\ell_2$ error &  TPR & FPR\\
	\hline
	Lasso &  59.83  & 0.51  & 0.49 \\
	LAD-Lasso & 124.49 &  0.49 & 0.43\\
	Extended Lasso & 16.17  & 0.36 & 0.20 \\
	ROMP  &46.47 &0.29 &0.18 \\
	{\bfseries Sparse-LTS} & 13.04 &  0.59 & 0.13 \\
	\belowspace
	{\bfseries Sparse-LTS-Ada} &  12.28  &0.63 & 0.19  \\
	\hline
	\end{tabular}
	%\end{tabular}
%\end{center}
\end{table}

